Towards Agentic Embodied Intelligence

Embodied Intelligence represents the ultimate frontier of bridging artificial intelligence with physical reality to achieve general-purpose physical agency. Recently, the infusion of multimodal foundation models has catalyzed an end-to-end sensorimotor paradigm, translating internet-scale semantic representations and human intents into motor actions. However, the prevailing monolithic paradigm treats continuous physical interaction as an unconstrained, open-loop sequence generation task. Consequently, it suffers from catastrophic compounding covariate drift, temporal attention dispersion over long horizons, and a complete absence of in-situ error recovery, fundamentally confining current systems to fragile, human-dependent conditional autonomy. We argue that transcending this plateau cannot be achieved by merely scaling feedforward policy weights; rather, the decisive breakthrough demands a fundamental paradigm shift toward Agentic Embodied Intelligence (AEI). In this survey, we examine embodied systems through an agentic lens, systematically characterizing the paradigm shift toward AEI across models, infrastructure, safety, data, environments, and evaluation. We formalize a cognitive closed loop: elucidating how physical grounding, deliberative planning, motor execution, and in-situ reflection dynamically interlock to bridge the chasm between abstract reasoning and continuous physical dynamics. Recognizing that the community remains in the nascent formative stage of building AEI, we critically dissect the prevailing open challenges across physical fidelity, real-time latency, and trustworthy deployment. We envision this work serving as a roadmap to guide future exploration toward resilient, general-purpose Physical AI in the open world.

==> resources/packages.tex <==
% For flexible citation formats (author-year, numeric)
\usepackage{natbib}

% For UTF-8 encoded CJK (Chinese, Japanese, Korean) characters
\usepackage{CJKutf8}

% 允许使用 \newcommandx
\usepackage{xargs}  

% 用于创建 todo notes
\usepackage{todonotes}  
% 用于表格multirow
\usepackage{multirow}

% 用于cref
\usepackage{cleveref}

\usepackage{amsmath}
\usepackage{dsfont}

% % using itemize
% \usepackage{enumerate}



\usepackage{svg}

\usepackage{mathrsfs}
\usepackage{adjustbox}
\usepackage{multirow}
\usepackage{multicol}
\usepackage{tcolorbox}
\usepackage{changepage}
\usepackage{enumitem}
\usepackage{graphicx}
\usepackage{amssymb}
\usepackage{xcolor}
\usepackage{float}
\usepackage{multirow}
\usepackage{threeparttable}
\usepackage{graphicx}
\usepackage{subcaption}
\usepackage{algorithm}
\usepackage{algpseudocode}
\usepackage{wrapfig}
\usepackage[table]{xcolor}  % loads xcolor with table support
\usepackage{colortbl}       % gives \columncolor, \rowcolor
\usepackage{tabularx} % Add to your preamble
\usepackage{makecell} % Add to your preamble
\usepackage[dvipsnames]{xcolor}
\usepackage{algorithm}

\newcolumntype{g}{>{\columncolor{gray!10}}c} % gray background
\newcommand{\KVSet}{\mathbf{KV}}
\newcommand{\ModelOuput}{\mathbf{X}_{\theta}}
\newcommand{\KVOutput}{\mathbf{kv}}

\definecolor{catgray}{gray}{0.9}
\definecolor{skyblue}{rgb}{0.53,0.81,0.92} % sky blue

% make it look transparent by mixing with white
\colorlet{skyblue!30}{skyblue!30!white} % 30% skyblue, 70% white

\definecolor{customblue}{RGB}{70,130,180}  % This is equivalent to rgb(70,130,180)

\newtcolorbox{evolbox}[2][]{%
  enhanced,
  % colframe=blue!70!black,
  colframe=customblue,
  colback=white,
  coltitle=white,
  rounded corners,
  boxrule=1pt,
  titlerule=0pt,
  toptitle=1mm,
  bottomtitle=1mm,
  fonttitle=\bfseries,
  % title=#3,
  % fontupper=\boxcontentfont\fontsize{10pt}{12pt}\selectfont,
  width=#2\textwidth, % This takes the second parameter as the width fraction
  % Applying the custom font with size
  % left=1mm, % Reduced left padding
  % right=1mm, % Reduced right padding
  % top=1mm, % Reduced top padding
  % bottom=1mm, % Reduced bottom padding
  #1
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\usepackage{minitoc}
\usepackage{url}

% cvpr packages
\PassOptionsToPackage{table,xcdraw}{xcolor}
\usepackage{titletoc}
\usepackage{placeins}
% 表格 ✔
\usepackage{pifont}

% \definecolor{cvprblue}{rgb}{0.21,0.49,0.74}
% \usepackage[pagebackref,breaklinks,colorlinks,allcolors=cvprblue]{hyperref}
\definecolor{RowBlue}{HTML}{E9F2FB}
\definecolor{RowRed}{HTML}{F9EAEA}
\definecolor{Top1}{HTML}{50DB4B} % 深绿
\definecolor{Top2}{HTML}{A5FFA2} % 中绿
\definecolor{Top3}{HTML}{D9FFD9} % 浅绿
\definecolor{Sub1}{HTML}{EAB8B8}
\definecolor{Sub2}{HTML}{E4E4E4}
\newcommand{\cmark}{\textcolor{green!60!black}{\checkmark}}
\newcommand{\xmark}{\textcolor{red!70!black}{\ding{55}}}

\newcommand{\dq}[1]{{\textcolor{cyan}{[DQ: #1]}}}
\newcommand{\myparagraph}[1]{\textbf{#1}\hspace{1.8ex}}

\renewcommand{\emph}[1]{\textit{#1}}


==> tab/3_passive2active.tex <==
\begin{table}[t]
\centering
\small
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.08}
\caption{\textbf{Questions and representative approaches for belief maintenance and information acquisition.} Works can support multiple functions; verification and stopping apply across acquisition mechanisms.}
\label{tab:perception-update-methods}
\begin{tabularx}{\linewidth}{
@{}
>{\raggedright\arraybackslash}p{0.35\linewidth}
>{\raggedright\arraybackslash}p{0.30\linewidth}
>{\raggedright\arraybackslash}X
@{}
}
\toprule
\textbf{Aspects}
& \textbf{Questions}
& \textbf{Approaches} \\
\midrule
\multicolumn{3}{@{}l}{\textit{Passive belief maintenance}} \\
\midrule
\rowcolor{AEIrow}
Correspondence and consistency
& How does new evidence connect to the stored scene?
& Hydra~\cite{hydra} \\
\addlinespace[2pt]
Change detection and temporal validity
& Which stored states must be revised?
& Khronos~\cite{khronos} \\
\addlinespace[2pt]
\rowcolor{AEIrow}
Task-conditioned evidence retrieval
& Which observations support the current query?
& 3D-Mem~\cite{3dmem} \\
\midrule
\multicolumn{3}{@{}l}{\textit{Active and interactive perception}} \\
\midrule
\rowcolor{AEIrow}
Viewpoint selection and targeted search
& Where should the robot observe next?
& VLFM~\cite{vlfm} \\
\addlinespace[2pt]
Physical probing and scene intervention
& Which interaction can reveal the hidden state?
& RoboEXP~\cite{roboexp} \\
\addlinespace[2pt]
\rowcolor{AEIrow}
Human clarification
& Which ambiguity should be resolved by asking?
& KnowNo~\cite{ren2023robotsask} \\
\addlinespace[2pt]
Verification and stopping
& Has the expected effect occurred?
& Code-as-Monitor~\cite{codeasmonitor} \\
& Is the evidence sufficient to answer?
& Explore-until-Confident~\cite{ren2024exploreconfident} \\
\bottomrule
\end{tabularx}
\end{table}
% \begin{table}[t]
% \centering
% \small
% \setlength{\tabcolsep}{4pt}
% \renewcommand{\arraystretch}{1.08}
% \caption{Questions and representative approaches for belief maintenance and information acquisition. Works can support multiple functions; verification and stopping apply across acquisition mechanisms.}
% \label{tab:perception-update-methods}
% \begin{tabularx}{\linewidth}{
% @{}
% >{\raggedright\arraybackslash}p{0.22\linewidth}
% >{\raggedright\arraybackslash}p{0.21\linewidth}
% >{\raggedright\arraybackslash}p{0.17\linewidth}
% >{\raggedright\arraybackslash}X
% @{}
% }
% \toprule
% \textbf{Aspect}
% & \textbf{Question}
% & \textbf{Representative work}
% & \textbf{Method summary} \\
% \midrule
% \multicolumn{4}{@{}l}{\textit{Passive belief maintenance}} \\
% \midrule
% Correspondence and consistency
% & How does new evidence connect to the stored scene?
% & Hydra~\cite{hydra}
% & Propagate loop-closure corrections through a layered scene graph. \\
% \addlinespace[2pt]
% Change detection and temporal validity
% & Which stored states must be revised?
% & Khronos~\cite{khronos}
% & Combine short-term motion tracking with long-term change estimation. \\
% \addlinespace[2pt]
% Task-conditioned evidence retrieval
% & Which observations support the current query?
% & 3D-Mem~\cite{3dmem}
% & Incrementally retain and retrieve informative multi-view snapshots. \\
% \midrule
% \multicolumn{4}{@{}l}{\textit{Active and interactive perception}} \\
% \midrule
% Viewpoint selection and targeted search
% & Where should the robot observe next?
% & VLFM~\cite{vlfm}
% & Rank exploration frontiers using a language-grounded value map. \\
% \addlinespace[2pt]
% Physical probing and scene intervention
% & Which interaction can reveal the hidden state?
% & RoboEXP~\cite{roboexp}
% & Select exploratory actions and build an action-conditioned scene graph. \\
% \addlinespace[2pt]
% Human clarification
% & Which ambiguity should be resolved by asking?
% & KnowNo~\cite{ren2023robotsask}
% & Use conformal prediction sets to trigger requests for help. \\
% \addlinespace[2pt]
% Verification and stopping
% & Has the expected effect occurred?
% & Code-as-Monitor~\cite{codeasmonitor}
% & Evaluate generated code for spatial and temporal constraints. \\
% & Is the evidence sufficient to answer?
% & Explore-until-Confident~\cite{explore}
% & Calibrate answer confidence to determine when exploration stops. \\
% \bottomrule
% \end{tabularx}
% \end{table}

